Automated Verification of Silq Quantum Programs using SMT Solvers

We present SilVer (Silq Verification), an automated tool for verifying behaviors of quantum programs written in Silq, which is a high-level programming language for quantum computing. The goal of the verification is to ensure correctness of the Silq quantum program against user-defined specifications using SMT solvers. We introduce a programming model that is based on a quantum RAM-style computer as an interface between Silq programs and SMT proof obligations, allowing for control of quantum operations using both classical and quantum conditions. Additionally, users can employ measurement flags within the specification to easily specify conditions that measurement results require to satisfy for being a valid behavior. We provide case studies on the verification of generating entangled states and multiple oracle-based algorithms.

==> Images/Silver-tikz.tex <==
\begin{tikzpicture}[
node distance=3cm and 1cm, font={\large},
squarednode/.style={rectangle, very thick, minimum size=5mm, align=center},
process/.style={draw=black,fill=orange!15,loosely dashed},
data/.style={draw=black,fill=violet!5},
pic/.style={inner sep=0pt}
]
%Nodes
\node[data] (silqprogram) [] {
\adjincludegraphics[width=.2\textwidth,trim={0 {.07\textwidth} 0 0},clip]{Images/silq.png}
};
\node[] (space) [right=of silqprogram] {};
\node[squarednode,data] (silspeq) [right=of space] {SilSpeq};
\node[squarednode, process] (silqinterpreter) [below=of silqprogram] {Syntax Tree\\Interpreter};
\node[squarednode,data] (intermediaterep) [below=of silqinterpreter] {Intermediate\\Representation};
\node[] (space2) [right=of intermediaterep] {};
\node[squarednode,process] (converter) [below=of space2] {Obligation Generator};
\node[squarednode,data] (programobl) [below left=3cm and -6cm of converter] {Program\\Obligations};
\node[squarednode,data] (speqobl) [right=of programobl] {Specification\\Obligations};
\node[squarednode,process] (Z3) [right= of speqobl] {
% \includegraphics[width=.1\textwidth]{Images/z3.png}
SMT\\Solver
};
\node[squarednode,draw=green] (unsat) [above right=-1cm and 3cm of Z3] {unsat$\implies$program correct $\checkmark$};
\node[squarednode,draw=red] (sat) [below right=-1cm and 3cm of Z3] {sat$\implies$counterexample$\cross$};

%Lines
\draw[line width=1pt,->] (silqprogram.south) -- node [right] {\hspace{1cm}syntax tree} (silqinterpreter.north);
\draw[line width=10pt,->] (silqinterpreter.south) -- (intermediaterep.north);
\draw[line width=10pt,->] (intermediaterep.east) -| (converter.north);
\draw[line width=10pt,->] (silspeq.south) -- node [align=left,right] {behaviour\\+ flags} ++(0,-13.6) -| (converter.north);
\draw[line width=10pt,->] (converter.south) -- ++(0,-1.25) -| (programobl.north);
\draw[line width=10pt,->] (converter.south) -- ++(0,-1.25) -| (speqobl.north);
\draw[line width=10pt,->] (programobl.south) -- ++(0,-2) -| (Z3.south);
\draw[line width=10pt,->] (speqobl.south) -- ++(0,-2) -| (Z3.south);
\draw[line width=10pt,->] (Z3.east) -- ++(1,0) |- (unsat.west);
\draw[line width=10pt,->] (Z3.east) -- ++(1,0) |- (sat.west);
\end{tikzpicture}

==> Images/program-ir.tex <==
% Source: https://tex.stackexchange.com/questions/103688/folded-paper-shape-tikz
\makeatletter
\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
% compute corner of ‘‘flipped page’’
\pgf@xc=\pgf@xb \advance\pgf@xc by-10pt % this should be a parameter
\pgf@yc=\pgf@yb \advance\pgf@yc by-10pt
% construct main path
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
}
}
\makeatother

\tikzstyle{doc}=[%
draw,
thick,
align=center,
color=black,
shape=document,
minimum width=20mm,
text width=50mm, 
minimum height=28.2mm,
inner sep=2ex,
]

\begin{tikzpicture}[scale=0.6, every node/.style={transform shape}]
  \node[doc] (silq) {Quantum Instruction\\Quantum Memory\\Classical Instruction\\Classical Memory\\Controls};
\end{tikzpicture}

==> Notes/goals.tex <==
\subsection{Goals}
Using SMART

Specific:


Measurable (write words/paragraphs/figures):


Achievable (rough draft, edit text, final version):
rough

Relevant (where section is):


Time-bound (write for x minutes):


\subsection{Action List}
\begin{enumerate}
    \item Confirm syntax for IR
    \item Discuss reasons why separate IR from SQIR and others
    \item Continue working on flags
    \item Develop a few simple examples in SilVer
\end{enumerate}

Note: Z3 v.4.8.17.0

==> Notes/unused.tex <==
\begin{figure}[th]
    \centering
    \begin{equation*}
    \begin{aligned}
        e_q ::= & x := const
        \vert x' := U(x)
    \end{aligned}
    \end{equation*}
    \caption{Silq-Unitary}
    \label{fig:silq-unitary}
\end{figure}

\begin{figure}[th]
    \centering
    \begin{equation*}
    \begin{aligned}
        e_c ::= & x
        \vert c
        \vert x := e_c
        \vert \textbf{return } x 
    \end{aligned}
    \end{equation*}
    \caption{Silq-Classical}
    \label{fig:silq-classical}
\end{figure}

==> Sections/Deprecated/conversion.tex <==
% In this section, we cover how Silq programs are converted into proof obligations.
For our Silq programs and \silspeq{} specifications, we convert each into an SMT encoding.
A Silq program is converted into our QRAM program model first, and then into \smtlib{} format.
We use $prog$ to denote a Silq program's SMT encoding.
\silspeq{} specifications can be directly converted into an SMT encoding, as mentioned in Section~\ref{sec:silspeq:expr}.
We use $pre$ and $post$ to represent a \silspeq{} specification's pre- and post-conditions SMT encoding respectively.

When a program is checked against its specification, the logical statement
\begin{equation}\label{SMTcheck}
    prog \land pre \land \lnot post
\end{equation}
is checked by an SMT solver, which looks for an execution (a model from $prog$), with pre-conditions given by $pre$, that does not satisfy the post-conditions, $post$, given by the user.
If conjunction~\eqref{SMTcheck} is satisfiable, then we have a possible program execution that does not meet the user defined specification.
However, if the conjunction is unsatisfiable and $prog \land pre$ is true for all states, then $\lnot post$ must be false and therefore $prog \land pre \land post$ must be true always.

% % Alternative using an algorithm environment
% \begin{algorithm}[t]
%     \label{alg:check}
%     \caption{How \silver{} checks program specification satisfaction, where $check(x)$ performs a satisfiability check of $x$ and returns $sat$, $unsat$ or $unkown$.}
%     \KwData{$pre, post, prog$}
%     \lIf{$check(prog) = unsat \lor check(pre \land post) = unsat$}{error}
%     \lIf{$check(prog) = unkown \lor check(pre \land post) = unkown$}{warning}
%     \lIf{$check(prog \land pre \land \lnot post) = unsat$}{\Return{unsat core}}
%     \lElseIf{$check(prog \land pre \land \lnot post) = unknown$}{\Return{reason}}
%     \lElse{\Return{model}}
% \end{algorithm}
% Algorithm~\ref{alg:check} shows how \silver{} checks the satisfaction of a program against a specification.
% The first two lines check that the specification and program themselves are satisfiable and returns an error or warning if not.
% Since $prog \land pre$ is true and if $check(prog \land pre \land \lnot post)$ returns false, it must be the case that $\lnot post$ is false and therefore $post$ is true; meaning that the program meets the specification.
% An unsat core can then be provided to the user to check.
% If the check is unkown, then the reason for it being unkown can be provided.
% Finally, if the check is satisfiable, then there is some program execution that violates the specification provided and a model is provided.

We focus on converting Silq programs into proof obligations, with particular focus on how conditional ($\textbf{if } e \textbf{ then } e_1 \textbf{ else } e_2$) and measurement ($\textbf{measure}$) statements, as well as flags, affect generation of proof obligations.

Throughout we use $[i, j)$ to denote the set $\{i, i+1, \dots, j-2, j - 1\}$ for $i < j$.

\subsection{\silqfrag{} to QRAM Program Model}
The formula for how \silqfrag{} expressions are converted into the QRAM program model described in Definition~\ref{def:qram} is given in Appendix~\ref{app:ir}.

\subsection{Conversion of QRAM Program Model into Proof Obligations}
We can think of the conversion as a function on the Processes in the QRAM program model into proof obligations.
Purely classical instructions, $\cinst$, are converted in a similar way as described in Section~\ref{sec:prelim:classicalverif}, where classical variables are represented by symbols at certain time steps of the computation.
The values of variables at later time steps are determined by the values of the same variable at an earlier time step.

The quantum state throughout the computation is represented by a vector of symbols whose (exponential) size is based on the sizes of the quantum variables throughout the program.
In a similar way to the classical obligations, there is a vector at each time step within the program.
Later quantum symbols have values that are based on obligations from older symbols.
Whilst costly, this representation is unavoidable as we need to track the full quantum state for model checking.
For example, a quantum memory consisting of
\begin{equation*}
\begin{aligned}
\memq(p) = (p, \size(p), V_p), & & \memq(r) = (r, \size(r), V_r)
\end{aligned}
\end{equation*}
is represented by the symbols
\begin{equation*}
    \mathrm{q}Q\mathrm{v}V_r|\mathrm{r}R\mathrm{v}V_r
\end{equation*}
where $Q \in [0, 2^{\size(q)})$ and $R \in [0, 2^{\size(r)})$.
As the program progresses, the versions of the quantum variables are updated each time they are operated upon.
We refer to the symbol vector representing the states of the quantum variables as the \emph{quantum state} throughout.

Initialising a new quantum variable, $\qinit$, expands the quantum state and quantum unitary operations, $\qop$, affect the quantum state using their matrix representation.\footnote{In our implementation, we include an Instruction that allows parallel unitary operations to occur in a single matrix, reducing the number of obligations generated.}
Measurement statements are converted into proof obligations that encapsulate the probabilities of measuring a variable in the quantum state and puts additional constraints on those probabilities depending on the flag used.
Additionally the quantum state is modified depending on what value is measured.


Conditional statements affect the program depending on whether the variable affected is classical or quantum.
A classical conditional acts in a similar way to how a classical program would be verified, whereas a quantum case requires the generation of a quantum gate to be applied to the quantum state.
Further discussion around how conversion of measurement and conditionals are handled is given in Appendix~\ref{app:convert}.

==> Sections/Deprecated/conversiontheory.tex <==
\subsection{Conditionals on Proof Obligations}
Throughout, we write $\tau(p)$ as the proof obligations generated for process $p$.
There are two types of controls we need to consider, classical and quantum.
Let $\ctrls_c$ and $\ctrls_q$ respectively denote the classical and quantum controls of a list of controls, $\ctrls$.
We analyse how each of these affect obligations.

% \begin{comment}
\paragraph{Classical}
The classical controls, $\ctrls_c$, determine if a block of code should be ran at all.
Consider the following Silq code:
\def\bbool{\mathrm{b}}
\def\xnat{\mathrm{x}}
\def\qqubit{\mathrm{q}}
% 
\begin{equation*}
\begin{minted}{d}
    if b {
        x = x + 2;
        q := X(q);
    }
\end{minted}
\end{equation*}
% 
where $\bbool$ is a boolean (0 or 1), $\xnat$ is a classical integer and $\qqubit$ is a variable referring to a qubit.
This is represented by the Program $(p_1, p_2)$, where
% 
\begin{equation*}
\begin{aligned}
    p_1 = & (\qcskip, \memq, \cop(x, size(x), \binary(x, +, 2)), \\
    & \memc[x \to (x size(x), 1)], (\binary(b, ==, 1))), \text{ and}\\
    p_2 = & (\qop(X, q), \memq[x \to (q, size(q), 1)], \qcskip, \\
    & \memc[x \to (x size(x), 1)], (\binary(b, ==,1))).
    \end{aligned}
\end{equation*}
% 
If $\bbool$ is true, then the code in the if block is ran changing the value of $\xnat$ and the quantum state.
However, if $\bbool$ is false, then the code is not ran and the values remain the same.

This means that when converting Programs to proof obligations, two types of obligations are generated.
The first type state that when $\bbool$ is true, then we update the new variable symbols in the way described by the operation.
The second type state that when $\bbool$ is false, then we set the new symbols to be the same as the previous symbols.
% For the example given, the proof obligations generated are
% \begin{equation*}
%     \begin{minted}[autogobble]{text}
%         if b: xv1 = xv0 + 2
%         if not b: xv1 = xv0
%         if b: q0v1 = q1v0
%         if b: q1v1 = q0v0
%         if not b: q0v1 = q0v0
%         if not b: q1v1 = q1v0.
%     \end{minted}
% \end{equation*}
Note that for quantum variables, the next quantum state needs to be set to be the same as the previous quantum state.

If $\ctrls_c = (b_1, \dots b_n)$, then we can include the individual boolean conditions in a logical and, $\bigwedge$, statement.
Therefore, proof obligations for classical conditionals work in a similar as to how one would do it classically
\begin{equation*}
\begin{aligned}
    & \tau((\qinst, \memq, \cinst, \memc, \ctrls)) = \\
    & \mathrm{if } \bigwedge_{b_i \in \ctrls_c} b_i: \tau((\qinst, \memq, \cinst, \memc, \ctrls_q) \\
    & \mathrm{if } \lnot (\bigwedge_{b_i \in \ctrls_c} b_i): \idproc((\qinst, \memq, \cinst, \memc, \ctrls_q)),
\end{aligned}
\end{equation*}
where $\idproc(p)$ sets any variables modified by process $p$ to be the same as their previous version.
% \end{comment}
% 
\paragraph{Quantum}
Quantum controls, $\ctrls_q$, only affect the quantum state of a program and should not affect classical variables.
This behaviour is already captured in Silq and so we do not need to discuss the change of classical variables.
Additionally, measurement cannot be controlled by a quantum variable as well.
Thus, we only need to consider Programs with quantum controls that only use $\qop$ operations.
These are generated by Silq statements such as
\begin{equation*}
    \begin{minted}[autogobble]{d}
    if r == 1{
        s := H(s);
    }
    \end{minted}
\end{equation*}

and so we only need to consider Processes of the form
\begin{equation*}
\begin{aligned}
    & (\qop(U, s), \memamend_q(s), \qcskip, \memc, (\op(r), \dots)).
\end{aligned}
\end{equation*}
For the example given $U = H$ and $\op(r) = \binary(r, ==, 1)$.

The quantum control acts as a control operator on a unitary gate for another quantum variable.
The unitary operation (within the conditional block) performed on the quantum state is modified depending on the quantum variable that is being controlled.

This modification to the unitary operation is computed in the following way.
Let $U'$ be the unitary operation that modifies the quantum variable $s$.
We write $U$ to be the quantum operation that applies $U'$ to $s$ and the identity operation $I$ on every other quantum variable.
Consider $\op(b(r))$ (in our list of controls $\ctrls_q$) which applies some boolean operation $b$ on a quantum variable $r$.
Let $S$ be the size of the quantum state.
For $v \in [0, 2^S)$, let $b_v \in \{0,1\}$ denote the result of applying $b$ to the value of $r$ in the quantum state with value $v$.
Create the matrix $B = \diag((b_v)_{v \in [0, 2^S)})$.
Then the controlled unitary operation is
\begin{equation}
    \label{eq:cucalc}
    CU = I_q + (U - I_q). B
\end{equation}
where $I_q$ is the identity operation on the quantum state.

If there are multiple quantum controls, $\ctrls_q = (\op(b^1(r_1)), \dots \op(b^n(r_n)))$, then one finds the vectors $(b^i_v)$ for each $1 \leq i \leq n$ and calculates $(b_v) = (\bigwedge_i b^i_v)$.
This new vector $b_v$ is then used in $B$ to calculate $CU$ as given in Equation~\eqref{eq:cucalc}.
Additionally, even though the example of $U$ provided only affects one quantum variable, $U$ can be replaced with a unitary operation that affects the entire quantum state apart from any control variables.

The proof obligations generated are
\begin{equation*}
    \begin{aligned}
    & \tau((\qop(r), \memq' = \memiter_{\memq}(r), \qcskip, \memc, \ctrls_q)) = \\
    & (\memq')_i = \sum_j CU_{ij} (\memq)_j \text{ for } i \in [0, 2^S),
    \end{aligned}
\end{equation*}
where $(\mem)$ denotes the quantum state (vector of symbols) for memory $\mem$.

\subsection{Proof Obligations from Measurement}
When generating the proof obligations for measurement, we have
\begin{equation*}
    \begin{aligned}
        & \tau((\qmeas(\varq), \memdel_{\memq}(\varq),
        \cmeas(\varc), \memamend_{\memc}(\varc), \ctrls)) = \\
        &
        \qquad
        \obsprob
        \land \obsmeas
        \land \obspost
    \end{aligned}    
\end{equation*}
where $\obsprob, \obsmeas$ and $\obspost$ are \emph{probability} \emph{measurement} and \emph{post-state} obligations respectively.
Within these obligations are restrictions on the measurement probabilities of values that a quantum variable can take.
Measurement probabilities are represented by symbols as $\mathrm{Pr\_q\_v}w\_i$ where $q$ is a quantum register/variable, $w$ is the current version and $i$ is the measured state.
Additionally the measured value of a register $q$ is represented by the symbol $\mathrm{meas\_}q$.

\paragraph{Probability Obligations}
The obligations generated by $\obsprob$ are obligations on the probability of measuring different values.
They simply state that the probability of any measurement value of the quantum state is between 0 and 1, calculate the values of the probabilities (based on the state measured) and that the sum of these probabilities is 1.
These are expressions from some of the formula in Section~\ref{sec:bg:quantum}.
% For example, measurement of a single qubit $q$ generates the obligations
% \begin{equation*}
%     \begin{minted}[autogobble]{text}
%         0 <= Pr_q_v0_0
%         Pr_q_v0_0 <= 1
%         0 <= Pr_q_v0_1
%         Pr_q_v0_1 <= 1
%         Pr_q_v0_0 + Pr_q_v0_1 = 1
%         Pr_q_v0_0 = |q_v0_0|^2
%         Pr_q_v0_1 = |q_v0_1|^2
%     \end{minted}
% \end{equation*}
% where $\mathrm{Pr\_q\_v}w\_i$ is the symbol representing the probability that measuring version $w$ of the quantum register $q$ results in the value $i$.

\paragraph{Measurement Obligations}
Obligations generated by $\obsmeas$ put restrictions on how and what can be measured.
These obligations are influenced by the Flags from \silspeq{} (as described in Section~\ref{sec:flags}):
a \rand{} flag puts no restrictions on measurement, \ie{}any value can be picked;
a \cert{} flag restricts the measured value such that values must have a measurement probability equal to 1, \ie{} $\mathrm{meas\_}q == i \implies \mathrm{Pr\_}q\mathrm{\_v}w\_i == 1$; and
\highprob{a} flags say that a measured value, $i$, can only be picked if its measurement probability is higher than the set value, \ie{} $\mathrm{meas\_}q == i \implies \mathrm{Pr\_}q\mathrm{\_v}w\_i \geq a$.

\paragraph{Post-state Obligations}
Post-state obligations determine the state after measurement and is calculated  for each possible measurement based on the formula at the end of Section~\ref{sec:bg:quantum}.

==> Sections/Deprecated/silspeq.tex <==
In this section, we introduce the language that we use for specifying behaviour for programs written in Silq.
\silspeq{} is designed in a way such that it is easy for the user to write specification that is easily translatable into SMT obligations.

\subsection{Defining Variables}
In \silspeq{}, the user defines variables before they are used.
Definitions require the user to provide a variable name and a type.
The types that variables can take are limited to integers of fixed bit size and functions of these types.
These are respectively represented by the following syntax
\begin{equation*}
    \langle type \rangle ::= \{0,1\}^n \mid \langle type \rangle \to \langle type \rangle,
\end{equation*}
where $n \in \mathbb{N}$.
A definition is then usually written as
\begin{equation*}
    \text{define } \langle name \rangle : \langle type \rangle.
\end{equation*}

When converted into SMT format, integers are represented as integers with obligations on the values they can take.
Functions are converted into functions on integers, with restrictions on their inputs and outputs.

\subsection{Expressions}
\label{sec:silspeq:expr}
\silspeq{} uses a combination of arithmetic and logical expressions, denoted $\alpha$ and $l$ respectively,

\begin{equation*}
    \begin{aligned}
    \alpha ::= & \; m \in \mathbb{Z} \mid var \mid f(\alpha_1) \mid \alpha_1 * \alpha_2 \mid \alpha_1 + \alpha_2 \mid \alpha_1^{\alpha_2} \mid (\alpha_1) \\
    l ::= & \; \ff \mid \alpha_1 = \alpha_2 \mid \alpha_1 < \alpha_2 \mid \lnot l_1 \mid l_1 \& l_2 \mid @ var. l
    \end{aligned}
\end{equation*}
where $var$ is a defined variable, $f$ is a defined function, $\ff$ denotes falsity ($\bot$), $\&$ represents logical and ($\land$), and $@$ represents for all ($\forall$).
Other arithmetic and logical expressions can be derived by combining the above (e.g. $-, /$ for arithmetic expressions and $\leq, >, \lor, \implies, \exists, \dots$ for logical expressions).

For convenience, in the implementation we include several useful expressions as shorthand for certain expressions.
For example, we write $a.b$ to denote the bitwise dot product of two integers with the same number of bits.
That is $a.b = \sum_{i=0}^{n-1} a_i b_i$ where $a_i, b_i$ are the bits of $n$-(qu)bit numbers $a, b$ respectively.\footnote{This summation can also be written as $\sum_{i=0}^{n-1} [(a / 2^i) (b/ 2^i) \mod{2}]$.}

In \silspeq{}, these expressions are wrapped in an assert statement:
\begin{equation*}
    \text{assert}(l).
\end{equation*}
Expressions can easily be converted into SMT format by using the appropriate SMT expression and referring to variables when needed.
Shorthand expressions, such as $a.b$, can also be converted using appropriate SMT expressions as well.

\subsection{Flags}
\label{sec:flags}
Many quantum verification frameworks perform measurement based on a conditional statement structure; \ie if a qubit is measured and the result is $\ket{1}$, perform one command, otherwise perform another.
In \silver{}, we instead consider the properties of measurement that we wish to verify as well.
For instance, some quantum programs may require certainty in any result that might be measured, whereas others may simply require the most likely result.

To achieve this we include \emph{flags} in the \silspeq{} function definition that tell us what property of measurement we wish to verify a given function.
This changes the measurement outcome that can occur.
Additionally this allows us to either restrict the cases we need to consider.
For instance, if we allow only measurement to be done with certainty, then the solver only needs to consider measurement values that satisfy measurement with certainty.
On the other hand, the flexibility of flags mean that the solver can consider all possible measurement values and take these into account as well.

Flags allow the user to specify certain approaches that should be taken when verifying Silq programs, changing the obligations that are generated from the intermediate representation.
For \silver{}, flags mainly affect measurement.
For numerous quantum algorithms, there are certain properties about measurement that we want to be able to verify.

The types of flags available are described below:
\begin{itemize}
    \item The \rand{} flag puts no obligations on measurement and so any measurement result is possible so long as it has a non-zero likelihood of occurring.
    \item The \cert{} flag specifies that for any run of the program, there must be a state that has a measurement probability of $1$, \ie with certainty.
    \item The $\highprob{x}$ (with high probability) flag states that for any run of the program, we only consider measurement results that occur with probability greater than $x$.
    For ease, we write $\emph{whp} = \highprob{0.5}$ and note that $\cert{} = \highprob{1}$.
\end{itemize}

% The \atval{} flag...

Flags interact with the obligations generated from measurement instructions ($\qmeas$ and $\cmeas$).
% We formally show how the obligations generated from measurement instructions are affected by flags in Section~\ref{sec:conversion}.

\subsection{Function Structure}
A \silspeq{} file is automatically generated by \silver{} if one does not exist.
This file contains each function written within the Silq file, along with its input arguments defined as a \silspeq{} type and an additional return argument that encapsulates the output of the function.
This return argument is denoted by $\langle\textit{function name}\rangle\_ret$.

Each function contains \emph{pre}- and \emph{post}-condition blocks.
While variables can be defined both in the pre- and post-condition blocks, statements that are true before the program is run should be defined in the pre-condition block and statements that are true after running the program should be defined in the post-condition block.

==> Sections/Deprecated/vir.tex <==
Before converting Silq programs directly into proof obligations, it is helpful to separate the quantum sections of code from the classical code while tracking the controls that affect either system. To this end, we introduce a symbolic intermediate representation for programs written in Silq.

Throughout, we assume a set of variable names, $\Vars$, and the size function, $\size(x)$, which gives the number of bits/qubits needed to represent $x$ is defined.
The size of variable $x$ can be found based on the type of $\var \in \Vars$.

\subsection{Instructions}
We begin by firstly introducing the quantum instructions, $\qinst$, that can be performed on the quantum part of the program.
\begin{definition}[\qinst]
A quantum instruction, $\qinst$, is defined as
\begin{equation*}
    \begin{aligned}
        \qinst ::= & \qcskip
        \\ \vert & \qinit(\var,n,c)
        \\ \vert & \qop(U,\var)
        \\ \vert & \qmeas(\var)
        % \\ \vert & \qpar(\Vec{U})
        ,
    \end{aligned}
\end{equation*}
where
$\var \in \Vars$,
$n$ is the size of the register ($\size(\var)$),
$c$ is a constant,
and
$U$ is an uncontrolled unitary operation.
% $\Vec{U}$ is a vector of unitary operations $U_i$ acting on different qubits or registers
\end{definition}
The commands are designed to be intuitive:
$\qcskip$ does nothing,
$\qinit$ initialises a new quantum register $x$ with $n$ qubits,
$\qop$ performs a unitary operation $U$ on a qubit or quantum register $x$,
and $\qmeas$ performs a measurement on a qubit or register $x$.
% and $\qpar$ performs multiple unitary operations, $\Vec{U}$, in parallel.

We now introduce the classical instructions, $\cinst$, that can be performed on the classical part of the program.
First, we introduce $\op$ instructions that encapsulate unary and binary operations.
\begin{definition}[$\op$]
An operation instruction, $\op$, is defined as
\begin{equation*}
    \begin{aligned}
        \op ::= & \unary(\diamond, a) \vert \binary(l, \star, r),
    \end{aligned}
\end{equation*}
where $\diamond$ is some unary operation, $\star$ is a binary operation and $a, l, r$ are arguments.
\end{definition}
Arguments can be variables $\var \in \Vars$ that have been defined previously or numbers.
The $\op$ instructions can be interpreted as performing $\diamond a$ for unary operations or $l \star r$ for binary operations.
For some operation, $b$, that is unary or binary, $\op(b)$ represents its appropriate symbolic instruction representation.
% Say OP(b) = ...; 

\begin{definition}[\cinst]
A classical instruction, $\cinst$, is defined as
\begin{equation*}
    \begin{aligned}
        \cinst ::= & \qcskip \\
        \vert & \cop(\var, s, const) \\
        \vert & \cop(\var, s,\op) \\
        \vert & \cmeas(\var) \\
        \vert & \return(\var),
    \end{aligned}
\end{equation*}
% \begin{grammar}
%     <classical-instruction> ::= \qcskip
%     \alt  \cop(\var, s, const)
%     \alt  \cop(\var, s,\op)
%     \alt  \cmeas(\var)
%     \alt \return(\var),
% \end{grammar}
where $const$ is a constant, $\var \in \Vars$ and $s = \size(x)$.
\end{definition}
The commands are interpreted as follows:
$\qcskip$ does nothing,
$\cop$ sets a variable, $\var$, to be a constant, $val$, or the result of an $\op$ instruction;
$\cmeas$ stores a measurement result in a classical variable $\var$;
and $\return$ returns the value of the classical variable $\var$.

Finally, we introduce the concept of control instructions, which are a restricted set of $\op$ instructions.
\begin{definition}[\ctrl]
A control instruction, $\ctrl$, is an $\op$ instruction that can use either classical or quantum variables in their argument and uses logical or comparison operators for their operation ($\lnot$, $\leq$, $==$, \dots...). 
\end{definition}
For example, a conditional statement $\textbf{if } x \leq 2 \textbf{ then } e$ will have a control instruction $\binary(x, \leq, 2)$, where $x$ is a previously defined variable.

\subsection{Memory}
Firstly, we define how we keep track of variables as a program advances.
\begin{definition}[Register]
    A register is a triple $\reg = (\var, s, ver)$ where $\var \in \Vars$, $s \in \mathbb{N}$ is the number of (qu)bits required and $ver \in \mathbb{N}$ is the version number.
\end{definition}
We keep track of the version of variables throughout the program since when converting into SMT format, we want to make obligations about a variable at certain time steps as the program advances.
The obligations we wish to make about a variable at the start of a program may differ from those at the end of the program.
It is helpful to define a collection of registers.
\begin{definition}[Memory]
    A memory $\mem$ is a mapping between variables and registers, where if $\var \in \Vars$ is a variable and $\reg$ is its associated register, then $\mem(\var) = \reg$.
\end{definition}
We use $\mem' = \mem[\var \to \reg]$ to denote $\mem'(\var') = \reg$ if $\var' = \var$ and $\mem'(\var') = \mem(\var')$ otherwise.

Whilst a memory is defined to take in any variable, we create two different memories for our intermediate representation.
These two memories are a classical memory and a quantum memory, denoted $\memc$ and $\memq$ respectively.
This allows us to clearly separate variables used to represent classical and quantum data.
Additionally, we define some operations that can be performed on a memory in Figure~\ref{fig:vir:memory-ops}.

\begin{figure}[t]
    \centering
    \begin{equation*}
    \begin{aligned}
        \memadd_\mem(\var) & = \mem[\var \to (\var, \size(x), 0)]
        \\
        \memiter_\mem(\var) & = \mem[\var \to (\var, \size(x), ver+1)]
        \\
        \memamend_\mem(\var) & =
        \begin{cases}
            \memiter_\mem(\var) & \text{if } \mem(\var) \neq () \\
            \memadd_\mem(\var) & \text{otherwise}
        \end{cases}
        \\
        \memdel_\mem(\var) & = \mem[\var \to ()]
    \end{aligned}
    \end{equation*}
    \caption{Some operations that can be performed on a memory $\mem$:
    $\memadd$ adds a new variable to $\mem$;
    $\memiter$ updates the version of a variable in $\mem$;
    and $\memdel$ removes a variable from $\mem$.}
    \label{fig:vir:memory-ops}
\end{figure}
Note that we track changes at the register level rather than the memory level.
This is because only a subset of the memory may change over time.
Therefore, it is more efficient to track variables and only update them when they are changed as this will lead to fewer proof obligations being generated.
    
\subsection{Processes and Programs}
We now combine our previously defined instructions and memory representation to give us a representation of a single expression.
\begin{definition}[QRAM Process]
A QRAM process is a quintuple
\begin{equation*}
\proc = (Q, \memq, C, \memc, \ctrls)    
\end{equation*}
where $Q$ is a quantum instruction; $C$ is a classical instruction; $\memq, \memc$ are quantum and classical memory respectively; and $\ctrls = (c_1, \dots, c_n)$ is a list of $\ctrl$ instructions.
\end{definition}
For simplicity we assume that only one instruction at a time, \ie{}at least one of $Q$ or $C$ is the $\qcskip$ instruction.
The only instance when this is not the case is when we have a $\qmeas$ and $\cmeas$ instruction together.

Now that we have processes representing expressions, we represent programs as a list of processes.
\begin{definition}[QRAM Program Model]
    \label{def:qram}
    A QRAM program model is a sequentially composed list of processes $\prog = (\proc_1, \proc_2, \dots, \proc_n)$ whose memories differ by up to one memory operation,
    \ie{}for all $i \in \{1,\dots,n-1\}$, $\mem_q^{i+1} = \mem_q^{i}$ or $\mem_q^{i+1} = f(\mem_q^{i})$ where $f$ is one of the operations given in Figure~\ref{fig:vir:memory-ops} and $\mem_q^{j}$ is the quantum memory for $\proc_j$ (similarly for classical memory $M_c^j$).
\end{definition}
